Whose Language Counts as High Quality? Measuring Language Ideologies in Text Data Selection

Language models increasingly rely on massive web dumps for diverse text data. However, these sources are rife with undesirable content. As such, resources like Wikipedia, books, and newswire often serve as anchors for automatically selecting web text most suitable for language modeling, a process typically referred to as quality filtering. Using a new dataset of U.S. high school newspaper articles -- written by students from across the country -- we investigate whose language is preferred by the quality filter used for GPT-3. We find that newspapers from larger schools, located in wealthier, educated, and urban ZIP codes are more likely to be classified as high quality. We then demonstrate that the filter's measurement of quality is unaligned with other sensible metrics, such as factuality or literary acclaim. We argue that privileging any corpus as high quality entails a language ideology, and more care is needed to construct training corpora for language models, with better transparency and justification for the inclusion or exclusion of various texts.

==> tables/counties.tex <==


\begin{table}[t]
\centering
\small
% \resizebox{\textwidth}{!}{
\begin{tabular}{lr}
\multicolumn{2}{c}{\emph{U.S. Counties (w/ \% Adult $\ge$ Bachelors)}} \\
\toprule
 \textbf{Highest} \phighquality  & \textbf{Lowest} \phighquality \\
\midrule 

Lewis and Clark, MT (53\%) & Liberty, TX (12\%) \\
Albany, NY (58\%) & Clarion, PA  (19\%) \\
Summit, UT (65\%)  & Bayfield, WI       (38\%) \\
Arlington, VA (81\%)   & Saint Francois, MO  (12\%)  \\
Madison, MS (63\%)   & Gregg, TX     (28\%)  \\
Bronx, NY (38\%)	     & Frederick, VA  (36\%) \\
Fairfax City, VA (66\%)  & Greenbrier, WV  (26\%)    \\
San Francisco, CA (51\%)  & Calhoun, AL (32\%)  \\
% Osceola, FL (25\%)      & Smyth, VA   (25\%)  \\
% Marin, CA   (67\%)      & Panola, TX  (15\%) \\
% Bristol, MA  (41\%)   & Midland, TX  (25\%) \\
% Washington, OR (44\%)   & Caribou, ID     (17\%) \\
% Leon, FL  (55\%)       & Lewis, WV   (23\%)  \\
% Union, NC (38\%)    & Alpena, MI  (30\%)  \\
% Middlesex, CT (44\%)   & Douglas, MO  (17\%) \\

\bottomrule
\end{tabular}

% }
\caption{Random sample of counties with the highest  ($\ge$ 90th percentile; left column) and lowest ($\le$ 10th percentile; right column) average quality scores according to \openaifilter. In parentheses, we display the average \% adults ($\ge$ 25 years old) that have at least a bachelors degree among all zipcodes in that county. The counties with the highest \phighquality~tend to contain (or are near to) the largest cities of their respective states, and/or are highly educated. The counties with lowest \phighquality~tend to be more rural and less educated.}
% \dallas{I thikn we could shorten this to like 6 rows; most people won't know the vast majority of these counties anyway}}
\label{tab:counties}
\end{table}


==> tables/dataset_stats.tex <==
\begin{table*}[t!]
\centering
\small
% \resizebox{\textwidth}{!}{
\begin{tabular}{llr}
\toprule
 \bf Domain & \bf Corpus &  \bf Metadata  \\
\midrule 

% \midrule[0.03em]




  \schoolnewspapers 
 & 1.6M news articles by U.S. students
& School \& County Demographics \\
\nationalnewspapers 
& X articles from online news outlets
&  Bias \& Factuality Ratings \\
\argumentativeessays 
& X essays from high school and university students.
& Essay prompts \\
 \literature      
& X books from Gutenberg and Books3
& Authors and Genres \\
 \reddit
& 474 subreddits, 80K comments each. 
& Subreddit topic and community features  \\

\bottomrule
\end{tabular}

% }
\caption{Domains that make up our evaluation corpus, including the metadata that we use to analyze document or population level exclusion patterns. \reddit~was extracted and obtained by a third party and made available on \url{pushshift.io}. \suchin{fill in details.}}
% \nascomment{should top row explain what's in parentheses (``Eval.'' like in the subheader for novel domains)?}}
\label{tab:datasets}
\end{table*}

==> tables/demographic_regression.tex <==
\begin{table}[t]
\centering
\small
% \resizebox{\textwidth}{!}{
\begin{tabular}{lcc}
 & \multicolumn{2}{c}{\phighquality} \\



% Intercept                  0.3165      0.003     97.240      0.000       0.310       0.323
% urban_top_30[T.True]       0.0193      0.009      2.165      0.031       0.002       0.037
% educational_attainment     0.0149      0.003      5.384      0.000       0.009       0.020
% income_per_capita          0.0067      0.002      3.341      0.001       0.003       0.011
% fte_teacher                0.0083      0.002      3.362      0.001       0.003       0.013


% Intercept                 -0.5241      0.041    -12.712      0.000      -0.605      -0.443
% urban_top_30[T.True]       0.0106      0.008      1.411      0.158      -0.004       0.025
% educational_attainment     0.0051      0.002      2.167      0.030       0.000       0.010
% income_per_capita         -0.0001      0.002     -0.087      0.931      -0.003       0.003
% fte_teacher                0.0056      0.002      2.692      0.007       0.002       0.010
% num_tokens                 0.1411      0.007     20.441      0.000       0.128       0.155
% student_life_category     -0.0082      0.002     -3.894      0.000      -0.012      -0.004
% clubs_category            -0.0056      0.002     -2.635      0.009      -0.010      -0.001
% op_ed_category             0.0009      0.002      0.520      0.603      -0.002       0.004
% news_category              0.0034      0.002      1.604      0.109      -0.001       0.008
% sports_category            0.0078      0.002      3.755      0.000       0.004       0.012
% announcements_category    -0.0043      0.002     -1.938      0.053      -0.009    5.46e-05


% \multicolumn{4}{c}{Dependent Variable: Mean \phighquality per school} & & \\
%  & & \multicolumn{4}{l}{Mean \phighquality} \\
%  & & \multicolumn{4}{l}{per school} \\
\toprule
 \bf Feature & \bf M1 &  \bf M2  \\
\midrule 
% \midrule[0.03em]
Intercept & $\phantom{-}$0.3162$^{***}$ & $\phantom{-}$0.3244$^{***}$ \\
\midrule
Mixed Race Students &  $\phantom{-}$0.0108$^{***}$ & $\phantom{-}$0.0053^{*}\phantom{{}^{**}}\\
\midrule
\# FTE Teachers &  $\phantom{-}$0.0055$^{***}$ & $\phantom{-}$0.0052^{**}\phantom{{}^{*}}\\
Per-Capita Income$^\dagger$  &  $\phantom{-}$0.0066$^{***}$ & $-$0.0006\phantom{{}^{***}} \\
Education$^\dagger$ &  $\phantom{-}$0.0054$^{***}$ & $\phantom{-}$0.0057$^{*}$\phantom{{}^{**}}\\
\midrule
Urban$^\dagger$  &  $\phantom{-}$0.0228$^{*}$\phantom{{}^{**}} & $\phantom{-}$0.0116\phantom{{}^{***}}\\
\midrule
Article Category &$-$&$\phantom{-}$0.0118$^{***}$\\
Num. Tokens &$-$&$\phantom{-}$0.0459$^{***}$ \\
%  News     &$-$& $\phantom{-}$0.0034\phantom{{}^{***}} \\
% Opinion   &$-$ & $\phantom{-}$0.0009\phantom{{}^{***}} \\
%  Sports   &$-$ &$\phantom{-}$0.0078^{***}  \\
% Clubs   &$-$ &$-$0.0056^{**}\phantom{{}^{*}} \\
% Student Life   & $-$&$-$0.0082^{***} \\
% Announcements   & $-$&$-$0.0043\phantom{{}^{***}}\\
% Number of Tokens  &$-$ & $\phantom{-}$0.1411$^{***}$\\
\midrule
 LL  & $\phantom{-}$1242.9\phantom{{}^{***}} & $\phantom{-}$1454.2\phantom{{}^{***}}\\
\bottomrule
\end{tabular}
% }
\caption{Ordinary Least Squares regression between \phighquality~and demographic  variables in the \schoolnewspapers dataset. The \openaifilter~tends to prefer content written by richer schools in urban areas of the U.S., who tend to have more mixed race students (M1). When accounting for textual features (M2), the number of full-time teachers in a school and county education level remains significant predictors. These wealth variables correlate strongly with racial and electoral predictors (See appendix for details). $^\dagger$ indicates features at the county level (instead of school level).  See appendix for model breakdown per categories.  $^*p <$ 0.05,  $^{**}p <$ 0.01,$^{***}p \approx$ 0.0}
% \nascomment{should top row explain what's in parentheses (``Eval.'' like in the subheader for novel domains)?}}
\label{tab:demographic_regression}
\end{table}

==> tables/hinds_madison.tex <==



\begin{table}[t]
\centering
\small
% \resizebox{\textwidth}{!}{
\begin{tabular}{llc}
\toprule
 & \bf Reddit Topic & \bf Average Quality Score  \\
\midrule 
& ~Art           &    0.05 \\ 
 \parbox[]{3pt}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\bf \textsc{Lowest}}}} & ~Arts/Writing   &   0.06 \\
& ~Fashion/Beauty  &  0.06 \\
& ~Cute             & 0.06 \\
& ~Economics        & 0.07 \\
\midrule
 \parbox[t]{3pt}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\bf \textsc{Highest }}}} & ~Meta          &    0.13 \\
& ~Science    &       0.14 \\
& ~News/Politics &     0.14 \\
& ~Conspiracy     &   0.14 \\
& ~Psychology     &   0.16 \\
\bottomrule
\end{tabular}

% }
\caption{Reddit conversations generally have very low quality, but the lowest scoring reddit topics are generally more personal, while the highest scoring topics tend to be more factual or political.}
% \nascomment{should top row explain what's in parentheses (``Eval.'' like in the subheader for novel domains)?}}
\label{tab:reddit_topics}
\end{table}


==> tables/lowest_laureates.tex <==



\begin{table}[t]
\centering
\small
% \resizebox{\textwidth}{!}{
\begin{tabular}{lc}
\toprule
 \bf Author & \bf Average Quality Score  \\
\midrule 

\bf \books & \bf 0.51\\
Seamus Heaney         & 0.43\\
Paul Heyse            & 0.43\\
Pearl S. Buck         & 0.43\\
Derek Walcott         & 0.41\\
Eugene O'Neill        & 0.40\\
John Galsworthy       & 0.39\\
Gerhart Hauptmann     & 0.39\\
Maurice Maeterlinck   & 0.39\\
Rabindranath Tagore   & 0.35\\
George Bernard Shaw   & 0.27\\
\bottomrule
\end{tabular}

% }
\caption{Nobel Prize laureates with the lowest average quality scores among their works. Most of these laureates write plays or poetry.}
% \nascomment{should top row explain what's in parentheses (``Eval.'' like in the subheader for novel domains)?}}
\label{tab:nobel}
\end{table}

==> tables/reddit_convos.tex <==



\begin{table}[t]
\centering
\small
% \resizebox{\textwidth}{!}{
\begin{tabular}{llc}
\toprule
 & \bf Reddit Topic & \bf Average Quality Score  \\
\midrule 
& ~Art           &    0.05 \\ 
 \parbox[]{3pt}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\bf \textsc{Lowest}}}} & ~Arts/Writing   &   0.06 \\
& ~Fashion/Beauty  &  0.06 \\
& ~Cute             & 0.06 \\
& ~Economics        & 0.07 \\
\midrule
 \parbox[t]{3pt}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\bf \textsc{Highest }}}} & ~Meta          &    0.13 \\
& ~Science    &       0.14 \\
& ~News/Politics &     0.14 \\
& ~Conspiracy     &   0.14 \\
& ~Psychology     &   0.16 \\
\bottomrule
\end{tabular}

% }
\caption{Reddit conversations generally have very low quality, but the lowest scoring reddit topics are generally more personal, while the highest scoring topics tend to be more factual or political.}
% \nascomment{should top row explain what's in parentheses (``Eval.'' like in the subheader for novel domains)?}}
\label{tab:reddit_topics}
\end{table}


==> tables/reddit_regression.tex <==
\begin{table}[t]
\centering
\small
% \resizebox{\textwidth}{!}{
\begin{tabular}{lcc}
 & \multicolumn{2}{c}{\phighquality} \\

% Intercept      0.1120      0.002     52.052      0.000       0.108       0.116
% num_subs       0.0536      0.008      6.476      0.000       0.037       0.070
% sub_ratio     -0.0299      0.006     -4.975      0.000      -0.042      -0.018
% density        0.0592      0.007      7.976      0.000       0.045       0.074
% loyalty       -0.0099      0.003     -3.774      0.000      -0.015      -0.005
% activity      -0.0113      0.006     -2.000      0.046      -0.022      -0.000
% f_score       -0.3678      0.052     -7.032      0.000      -0.471      -0.265

% Intercept                         0.0531      0.003     15.270      0.000       0.046       0.060
% topic_highest_quality[T.True]     0.0149      0.003      5.789      0.000       0.010       0.020
% num_subs                          0.0740      0.006     11.772      0.000       0.062       0.086
% sub_ratio                        -0.0534      0.005    -11.235      0.000      -0.063      -0.044
% density                           0.0697      0.006     12.562      0.000       0.059       0.081
% loyalty                          -0.0157      0.002     -8.125      0.000      -0.019      -0.012
% activity                         -0.0205      0.004     -4.994      0.000      -0.029      -0.012
% f_score                          -0.1063      0.040     -2.682      0.008      -0.184      -0.028
% num_tokens                        0.0012   6.87e-05     17.779      0.000       0.001       0.001


% \multicolumn{4}{c}{Dependent Variable: Mean \phighquality per school} & & \\
%  & & \multicolumn{4}{l}{Mean \phighquality} \\
%  & & \multicolumn{4}{l}{per school} \\
\toprule
\bf Feature & \bf M1 & \bf M2 \\
\midrule 
% \midrule[0.03em]
Intercept  &  $\phantom{-}$0.1120$^{***}$ & $\phantom{-}$0.0531^{***}$\\
\midrule
Number of Subscribers & $\phantom{-}$0.0536$^{***}$ & $-$0.0740\phantom{{}^{***}} \\
Subscribers:Commenters & $-$0.0299$^{***}$ & $-$0.0534^{***}$ \\
User Loyalty &  $-$0.0099$^{***}$ &  $-$0.0157^{***}$\\
User Activity  &  $-$0.0113$^{*}$\phantom{{}^{**}} &  $-$0.0205$^{***}$\\
User Density  &  $\phantom{-}$0.0592$^{***}$ & \phantom{-}                          0.0697$^{***}$\\
\midrule
\mathcal{F}-Score & $-$0.3678$^{***}$ & $-$0.1063$^{***}$\\
\midrule
Topic     &$-$& \phantom{-}0.0149$^{***}$ \\
Number of Tokens  &$-$ & \phantom{-}0.0012$^{***}$\\
\midrule
 LL  & \phantom{-}1020.6\phantom{{}^{***}} & \phantom{-}1166.1\phantom{{}^{***}}\\
\bottomrule
\vspace{1mm}
& \multicolumn{2}{c}{$^*p <$ 0.05,  $^{**}p <$ 0.005,} \\
& \multicolumn{2}{c}{$^{***}p \approx$ 0.0} 
\end{tabular}
% }
\caption{Ordinary Least Squares regression between \phighquality~and metrics of community-specific language in Reddit comments. The \openaifilter~tends to prefer content written in larger, more mainstream subreddits with less user loyalty and activity and community-specific language (F-score). When controlling for the topic and the average number of tokens in a subreddit, most community-specific language metrics remain very significant.}
% \nascomment{should top row explain what's in parentheses (``Eval.'' like in the subheader for novel domains)?}}
\label{tab:reddit_ols}
\end{table}

==> tables/regression_new.tex <==
\begin{table}[t]
\centering
\small
% \resizebox{\textwidth}{!}{
\begin{tabular}{rlcc}
%  & \multicolumn{2}{c}{\phighquality} \\



% Intercept                  0.3165      0.003     97.240      0.000       0.310       0.323
% urban_top_30[T.True]       0.0193      0.009      2.165      0.031       0.002       0.037
% educational_attainment     0.0149      0.003      5.384      0.000       0.009       0.020
% income_per_capita          0.0067      0.002      3.341      0.001       0.003       0.011
% fte_teacher                0.0083      0.002      3.362      0.001       0.003       0.013


% Intercept                 -0.5241      0.041    -12.712      0.000      -0.605      -0.443
% urban_top_30[T.True]       0.0106      0.008      1.411      0.158      -0.004       0.025
% educational_attainment     0.0051      0.002      2.167      0.030       0.000       0.010
% income_per_capita         -0.0001      0.002     -0.087      0.931      -0.003       0.003
% fte_teacher                0.0056      0.002      2.692      0.007       0.002       0.010
% num_tokens                 0.1411      0.007     20.441      0.000       0.128       0.155
% student_life_category     -0.0082      0.002     -3.894      0.000      -0.012      -0.004
% clubs_category            -0.0056      0.002     -2.635      0.009      -0.010      -0.001
% op_ed_category             0.0009      0.002      0.520      0.603      -0.002       0.004
% news_category              0.0034      0.002      1.604      0.109      -0.001       0.008
% sports_category            0.0078      0.002      3.755      0.000       0.004       0.012
% announcements_category    -0.0043      0.002     -1.938      0.053      -0.009    5.46e-05


\multicolumn{4}{c}{\emph{Dep. Variable:} \phighquality, \emph{Num. Observations:} 1547}  \\
%  & & \multicolumn{4}{l}{Mean \phighquality} \\
%  & & \multicolumn{4}{l}{per school} \\
\toprule
 & \bf Feature & \bf Coefficient & \bf adj. $R^2$  \\
\midrule 
% \midrule[0.03em]
\multirow{5}*{\bf M1} &\emph{Intercept} & $\phantom{-}$0.3191$^{***}$ & \multirow{5}*{\emph{0.107}}\\
& Black &  $-$0.0002$^{\phantom{***}} \\
& White^{\circ} &  $\phantom{-}$0.0069$^{***}\\
& Indigenous  &  $-$0.0051$^{*{\phantom{**}}}$ \\
& Asian^{\circ}  &  $\phantom{-}$0.0278$^{***}$  \\
\midrule

\multirow{2}*{\bf M2} & \emph{Intercept} & $\phantom{-}$0.3191$^{***}$ & \multirow{2}*{\emph{0.079}} \\
& Median Home Value^{\circ} &  $\phantom{-}$0.0233$^{***}$\\
\midrule

\multirow{3}*{\bf M3} & \emph{Intercept} & $\phantom{-}$0.3191$^{***}$ & \multirow{3}*{\emph{0.112}} \\
& Adults $\ge$ Bachelors^{\circ} &  $\phantom{-}$0.0351$^{***}$\\
& Adults $\le$ High School &  $-$0.0177$^{***}$\\
\midrule
\multirow{3}*{\bf M4} & \emph{Intercept} & $\phantom{-}$0.3079$^{***}$ & \multirow{3}*{\emph{0.063}} \\
& Population Density^{\circ} &  $\phantom{-}$0.0107$^{***}$\\
& Num. Public Schools$^\dagger$^{\circ} & $\phantom{-}$0.0049$^{\phantom{***}}$ \\
\midrule

\multirow{3}*{\bf M5}  & \emph{Intercept} & $\phantom{-}$0.3200^{***}$  & \multirow{3}*{\emph{0.048}}\\
& Urban$^\dagger$^{\circ}  &  $\phantom{-}$0.0221$^{***}$\\
& Rural$^\dagger$^{\circ}  &  $-$0.0249$^{***}$ \\
\midrule

\multirow{2}*{\bf M6} & \emph{Intercept} & $\phantom{-}$0.3191^{***}$ & \multirow{2}*{\emph{0.091}} \\
& 2016 GOP Vote Share$^\dagger$^{\circ}  &  $-$0.0250$^{***}$ \\
% \midrule
% \multirow{3}*{\bf M7} & \emph{Intercept} & $\phantom{-}$0.3295$^{***}$& \multirow{3}*{\emph{0.382}} \\
% & Article Category &$\phantom{-}$0.0074$^{***}$\\
% & Num. Tokens &$\phantom{-}$0.0508$^{***}$ \\
\bottomrule
\end{tabular}
% }
\caption{Regression of the average \phighquality within a ZIP code in the \schoolnewspapers~dataset, on  demographic  variables. We observe \openaifilter~tends to prefer content written by richer schools in urban areas of the U.S. $^\dagger$ indicates features at the county level (instead of zipcode level), and $^{\circ}$ indicates features that remain statistically significant ($p <$ 0.05) in a global model that includes all demographic variables. $^*p <$ 0.05,  $^{**}p <$ 0.01,$^{***}p \approx$ 0.0}
% \nascomment{should top row explain what's in parentheses (``Eval.'' like in the subheader for novel domains)?}}
\label{tab:main_regression}
\end{table}

==> tables/regressions.tex <==
\begin{table}[t]
\centering
\small
% \resizebox{\textwidth}{!}{
\begin{tabular}{rlcc}
%  & \multicolumn{2}{c}{\phighquality} \\



% Intercept                  0.3165      0.003     97.240      0.000       0.310       0.323
% urban_top_30[T.True]       0.0193      0.009      2.165      0.031       0.002       0.037
% educational_attainment     0.0149      0.003      5.384      0.000       0.009       0.020
% income_per_capita          0.0067      0.002      3.341      0.001       0.003       0.011
% fte_teacher                0.0083      0.002      3.362      0.001       0.003       0.013


% Intercept                 -0.5241      0.041    -12.712      0.000      -0.605      -0.443
% urban_top_30[T.True]       0.0106      0.008      1.411      0.158      -0.004       0.025
% educational_attainment     0.0051      0.002      2.167      0.030       0.000       0.010
% income_per_capita         -0.0001      0.002     -0.087      0.931      -0.003       0.003
% fte_teacher                0.0056      0.002      2.692      0.007       0.002       0.010
% num_tokens                 0.1411      0.007     20.441      0.000       0.128       0.155
% student_life_category     -0.0082      0.002     -3.894      0.000      -0.012      -0.004
% clubs_category            -0.0056      0.002     -2.635      0.009      -0.010      -0.001
% op_ed_category             0.0009      0.002      0.520      0.603      -0.002       0.004
% news_category              0.0034      0.002      1.604      0.109      -0.001       0.008
% sports_category            0.0078      0.002      3.755      0.000       0.004       0.012
% announcements_category    -0.0043      0.002     -1.938      0.053      -0.009    5.46e-05


 & \multicolumn{3}{c}{\emph{Output:} \phighquality}  \\
%  & & \multicolumn{4}{l}{Mean \phighquality} \\
%  & & \multicolumn{4}{l}{per school} \\
\toprule
 & \bf Feature & \bf Coefficient & \bf LL  \\
\midrule 
% \midrule[0.03em]
\multirow{6}*{\bf M1} &\emph{Intercept} & $\phantom{-}$0.3295$^{***}$ & \multirow{6}*{\emph{1334.2}}\\
& Black &  $-$0.0082$^{**\phantom{*}} \\
& White^{\circ} &  $-$0.0065$^{*{\phantom{**}}}\\
& Hispanic^{\circ} & $-$0.0105^{**{\phantom{*}}}$ \\
& Indigenous  &  $\phantom{-}$0.0033$^{{\phantom{***}}}$ \\
& Asian^{\circ}  &  $\phantom{-}$0.0254$^{***}$  \\
& Mixed &  $\phantom{-}$0.0018$^{{\phantom{***}}}$ \\
\midrule
\multirow{4}*{\bf M2} & \emph{Intercept} & $\phantom{-}$0.3079$^{***}$ & \multirow{4}*{\emph{1357.6}} \\
& \# FTE Teachers^{\circ} &  $\phantom{-}$0.0107$^{***}$\\
& Per-Capita Income$^\dagger$  &  $\phantom{-}$0.0095$^{***}$  \\
& Education$^\dagger$ &  $\phantom{-}$0.0080$^{**}\phantom{{}^{*}} \\
& Num. Public Schools$^\dagger$^{\circ} & $\phantom{-}$0.0116$^{***}$ \\
\midrule
\multirow{3}*{\bf M3}  & \emph{Intercept} & $\phantom{-}$0.3331^{***}$  & \multirow{3}*{\emph{1330.1}}\\
& Urban$^\dagger$^{\circ}  &  $\phantom{-}$0.0221$^{***}$\\
& Rural$^\dagger$^{\circ}  &  $-$0.0341$^{***}$ \\
\midrule
\multirow{2}*{\bf M4} & \emph{Intercept} & $\phantom{-}$0.3295^{***}$ & \multirow{2}*{\emph{1334.2}} \\
& 2020 GOP Vote Share$^\dagger$^{\circ}  &  $-$0.0230$^{***}$ \\
\midrule
\multirow{3}*{\bf M5} & \emph{Intercept} & $\phantom{-}$0.3295$^{***}$& \multirow{3}*{\emph{1559.2}} \\
& Article Category &$\phantom{-}$0.0045$^{*\phantom{**}}$\\
& Num. Tokens &$\phantom{-}$0.0522$^{***}$ \\
\bottomrule
\end{tabular}
% }
\caption{\suchin{update table to reflect new results} Ordinary Least Squares regression between  demographic  variables in the \schoolnewspapers~dataset and the average \phighquality of a zipcode. We observe \openaifilter~tends to prefer content written by richer schools in urban areas of the U.S. $^\dagger$ indicates features at the county level (instead of zipcode level), and $^{\circ}$ indicates features that remain statistically significant ($p <$ 0.05) when combining their model with textual features. $^*p <$ 0.05,  $^{**}p <$ 0.01,$^{***}p \approx$ 0.0}
% \nascomment{should top row explain what's in parentheses (``Eval.'' like in the subheader for novel domains)?}}
\label{tab:main_regression}
\end{table}

==> tables/regressions_final.tex <==
\begin{table}[t!]
\centering
\small
% \resizebox{\textwidth}{!}{
\begin{tabular}{ll}
%  & \multicolumn{2}{c}{\phighquality} \\



\multicolumn{2}{c}{\emph{Dep. Variable:}\phighquality } \\
\multicolumn{2}{c}{  \emph{Num. Observations:} 1328}  \\
\multicolumn{2}{c}{  $R^2$: 0.133, Adj. $R^2$: 0.124}  \\

%  & & \multicolumn{4}{l}{Mean \phighquality} \\
%  & & \multicolumn{4}{l}{per school} \\
\toprule
 \bf Feature & \bf Coefficient \\
\midrule 
% \midrule[0.03em]
 \emph{Intercept} & $\phantom{-}$0.3229$^{***}$ \\
 \% Black Students &  $-$0.0024^{\phantom{***}} \\
 \% Asian Students &  $\phantom{-}$0.0085^{*\phantom{**}} \\
 \% Native Students &  $-$0.0014^{\phantom{***}} \\
 \% Pacific Isl. Students &  $\phantom{-}$0.0001$^\phantom{***}$\\
 \% Mixed Students &  $\phantom{-}$0.0049^$\phantom{***}$ \\
 \% Hispanic Students  &  $-$0.0006$^{\phantom{***}}$  \\
 \% Charter Schools &  $\phantom{-}$0.0008$^{\phantom{***}}$\\
 \% Private Schools &  $\phantom{-}$0.0037$^{\phantom{***}}$\\
 \% Magnet Schools &  $-$0.0006^{\phantom{***}}\\
  Median Home Value &  $\phantom{-}$0.0035$^{\phantom{***}}$\\
 \% Adults $\ge$ Bachelors &  $\phantom{-}$0.0129$^{***}$\\
 Population Density &  $\phantom{-}$0.0085$^{***}$\\
 School Size &  $\phantom{-}$0.0077$^{***}$\\
 Student/Teacher Ratio &  $-$0.0043\\

% \multirow{2}*{\bf M6} & \emph{Intercept} & $\phantom{-}$0.3191^{***}$ & \multirow{2}*{\emph{0.091}} \\
% & 2016 GOP Vote Share$^\dagger$^{\circ}  &  $-$0.0250$^{***}$ \\
% \midrule
% \multirow{3}*{\bf M7} & \emph{Intercept} & $\phantom{-}$0.3295$^{***}$& \multirow{3}*{\emph{0.382}} \\
% & Article Category &$\phantom{-}$0.0074$^{***}$\\
% & Num. Tokens &$\phantom{-}$0.0508$^{***}$ \\
\bottomrule
\end{tabular}
% }
\caption{Regression of the average \phighquality within a ZIP code in the \schoolnewspapers~dataset, on  demographic  variables. Larger, better resourced schools in urban, educated, (and to some extent wealthier) areas of the U.S tend to be scored higher by \openaifilter. $^\dagger$ indicates features at the county level (instead of zipcode level), and $^{\circ}$ indicates features that remain statistically significant ($p <$ 0.05) in a global model that includes all demographic variables. $^*p <$ 0.05,  $^{**}p <$ 0.01,$^{***}p \approx$ 0.0}
% \nascomment{should top row explain what's in parentheses (``Eval.'' like in the subheader for novel domains)?}}
\label{tab:main_regression}
\end{table}

==> tables/school_level_only_regression.tex <==
\begin{table}[t!]
\centering
\small
% \resizebox{\textwidth}{!}{
\begin{tabular}{lc}
%  & \multicolumn{2}{c}{\phighquality} \\



\multicolumn{2}{c}{Dependent variable: \phighquality } \\
\multicolumn{2}{c}{Observations: 1379 schools}  \\

%  & & \multicolumn{4}{l}{Mean \phighquality} \\
%  & & \multicolumn{4}{l}{per school} \\
\toprule
 \bf Feature & \bf Coefficient \\
\midrule 
% \midrule[0.03em]
 \emph{Intercept} & $\phantom{-}$0.3148$^{***}$\\
 
 Is Charter & $\phantom{-}$0.0472$^{***}$ \\
 Is Private &  $-$0.0045$^{\phantom{***}}$ \\
 Is Magnet &  $\phantom{-}$0.0211^{*\phantom{**}}   \\
  
  \% Black Students &  $-$0.0004^{\phantom{***}} \\
 \% Asian Students & $\phantom{-}$0.0136^{***} \\
 \% Native Students &   $-$0.0021^{\phantom{***}}  \\
 \% Pacific Isl. Students &  $-$0.0014$^\phantom{***}$ \\
 \% Mixed Students &  $\phantom{-}$0.0028$^{\phantom{***}}$  \\
 \% Hispanic Students &  $-$0.0022$^{\phantom{***}}$ \\
 Student:Teacher &    $-$0.0052^{\phantom{***}} \\
 School Size &   $\phantom{-}$0.0137^{***} \\
 \midrule
 $R^2$ & $\phantom{-}$0.071^{\phantom{***}} \\
 adj. $R^2$ & $\phantom{-}$0.064^{\phantom{***}}  \\

% \multirow{2}*{\bf M6} & \emph{Intercept} & $\phantom{-}$0.3191^{***}$ & \multirow{2}*{\emph{0.091}} \\
% & 2016 GOP Vote Share$^\dagger$^{\circ}  &  $-$0.0250$^{***}$ \\
% \midrule
% \multirow{3}*{\bf M7} & \emph{Intercept} & $\phantom{-}$0.3295$^{***}$& \multirow{3}*{\emph{0.382}} \\
% & Article Category &$\phantom{-}$0.0074$^{***}$\\
% & Num. Tokens &$\phantom{-}$0.0508$^{***}$ \\
\bottomrule
\end{tabular}
% }
\caption{Regression of the average \phighquality~of a school in the \schoolnewspapers~dataset, on  school-level demographic  variables only. We observe consistent findings with our main regression here: larger schools with more Asian students tend to be scored higher by \openaifilter. We also observe here that charter schools and magnet schools tend to have higher quality scores. $^*p <$ 0.05,  $^{**}p <$ 0.01, $^{***}p <$ 0.001. \dallas{needs updating}}
% \nascomment{should top row explain what's in parentheses (``Eval.'' like in the subheader for novel domains)?}}
\label{tab:school_level_only_regression}
\end{table}

==> tables/school_newspapers.tex <==
\begin{table}[t!]
\centering
\small
% \resizebox{\textwidth}{!}{
\begin{tabular}{cccc}
\toprule
\bf  Articles & \bf Schools & \bf Zipcodes  & \bf States/Terr. \\
 1.1M & 1.9K  & 1.8K  & 52   \\
\bottomrule
\end{tabular}

% }
\caption{Basic statistics of our \schoolnewspapers~dataset, which covers articles written by middle school, high school, and college students across the United States. We additionally gather demographic information associated with each school's zipcode or county using the Census. See Appendix for datasheet. \dallas{We could probably fit this into one-column if we drop one of the columns (maybe Counties?)} \dallas{Oh, also -- we probably shouldn't have 52 states, lol. Not sure that represents DC or PR or what but might want to check to see what's going on there}\suchin{yeah it's DC /PR haha. I'll make it States/Territories! }
}
% \nascomment{should top row explain what's in parentheses (``Eval.'' like in the subheader for novel domains)?}}

\label{tab:school_newspapers}
\end{table}
